A Machine Learning Approach to the Nirenberg Problem

This work introduces the Nirenberg Neural Network: a numerical approach to the Nirenberg problem of prescribing Gaussian curvature on $S^2$ for metrics that are pointwise conformal to the round metric. Our mesh-free physics-informed neural network (PINN) approach directly parametrises the conformal factor globally and is trained with a geometry-aware loss enforcing the curvature equation. Additional consistency checks were performed via the Gauss-Bonnet theorem, and spherical-harmonic expansions were fit to the learnt models to provide interpretability. For prescribed curvatures with known realisability, the neural network achieves very low losses ($10^{-7} - 10^{-10}$), while unrealisable curvatures yield significantly higher losses. This distinction enables the assessment of unknown cases, separating likely realisable functions from non-realisable ones. The current capabilities of the Nirenberg Neural Network demonstrate that neural solvers can serve as exploratory tools in geometric analysis, offering a quantitative computational perspective on longstanding existence questions.

==> schematic.tex <==
\usetikzlibrary{arrows.meta, positioning, calc}

\begin{tikzpicture}[>=Stealth, node distance=2.5cm]
  \node (xy) {$(x, y)$};
  \node (xyz) [right=of xy] {$(X, Y, Z)$};
  \node (u) [right=of xyz] {$u$};
  \node (g) [right=of u] {$g(x,y)$};
  \node (g0) [below=1.2cm of xy] {$g_0(x,y)$};
  
  
  \draw[->] (xy) -- node[above] {$T$} (xyz);
  \draw[->] (xyz) -- node[above] {NN} (u);
  \draw[->] (u) -- node[above] {$e^u g_0$} (g);

  \draw[->] (xy) -- (g0);

\coordinate (ug_mp) at ($(u)!0.5!(g)$);
\coordinate (below_ug) at ($(ug_mp |- g0)$);

\draw[->] (g0) -- (below_ug) -- (ug_mp);


\end{tikzpicture}


